Endorsing Titanium-Scandium Radionuclide Generator for PET and Positronium Imaging

The development of PET and positronium imaging techniques is strictly related to the availability of suitable radionuclides and robust radiochemistry platforms. Among the emerging candidates, $^{44}$Sc has attracted significant interest due to its favourable physical properties, including a half-life of $\sim$4 hours, a pure $\beta^{+}$ emission profile, and the additional prompt $\gamma$-emission that enables advanced triple-photon detection schemes. These characteristics make $^{44}$Sc particularly promising for highresolution imaging and novel quantitative methodologies. However, routine clinical and preclinical implementation requires a practical, sustainable, and cost-efficient production route. In this context, we propose a titanium-scandium radionuclide generator as an optimal solution. This study focuses on optimising the synthesis of the long-lived parent isotope, $^{44}$Ti ($T_{1/2}$ = 59.1 years), from which $^{44}$Sc can be selectively eluted in a chemically pure form when needed. An analysis of various production pathways was conducted, including proton and deuteron reactions on scandium, as well as $\alpha$-particle and lithium-induced reactions on calcium, to determine the most efficient reaction parameters, target design, and expected yield. Furthermore, we identify some existing cyclotron facilities suitable for implementing this technology. Results indicate that efficient $^{44}$Ti production is achievable using proton beams in the 20-30 MeV range under extended irradiation conditions. The proposed generator system would enable routine and decentralised $^{44}$Sc supply. Its integration with the novel J-PET scanner may significantly reduce diagnostic costs and improve access to advanced PET imaging in regions with limited medical imaging infrastructure.

==> mystyle.tex <==
\usepackage{ragged2e}
\makeatletter

% -----------------------------------------------------------------------------
% Section formatting
% -----------------------------------------------------------------------------
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}

\renewcommand\p@subsection{}

\renewcommand{\section}{\@startsection{section}{1}{\z@}%
  {-5ex \@plus -1ex \@minus -.2ex}%
  {5ex \@plus.2ex}%
  {\centering\normalfont\bfseries}}

\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}%
  {-5ex \@plus -1ex \@minus -.2ex}%
  {5ex \@plus.2ex}%
  {\centering\normalfont\normalsize}}


% -----------------------------------------------------------------------------
% Captions
% -----------------------------------------------------------------------------
\renewcommand{\thetable}{\Roman{table}} % Roman numerals for tables

% Redefine labels
\renewcommand{\fnum@table}{TABLE~\thetable}
\renewcommand{\fnum@figure}{Fig.~\thefigure.}

% Custom caption for tables
\newcommand{\APPA@tabcap}[2]{%
  \noindent\makebox[\linewidth][r]{#1}\par\vspace{0.5ex}%
  \small\parbox{\linewidth}{\justifying\noindent #2}}

% Custom caption for figures
\newcommand{\APPA@figcap}[2]{%
  \small\parbox{\linewidth}{\justifying\noindent #1\ #2}}

% Master caption builder
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \begingroup
    \edef\APPA@captype{\@captype}%
    \expandafter\ifx\csname fnum@\APPA@captype\endcsname\fnum@table
      \APPA@tabcap{#1}{#2}%
    \else
      \APPA@figcap{#1}{#2}%
    \fi
  \endgroup
  \vskip\belowcaptionskip}
\makeatother

\makeatother
